Designing Reconfigurable Intelligent Systems with Markov Blankets

Compute Continuum (CC) systems comprise a vast number of devices distributed over computational tiers. Evaluating business requirements, i.e., Service Level Objectives (SLOs), requires collecting data from all those devices; if SLOs are violated, devices must be reconfigured to ensure correct operation. If done centrally, this dramatically increases the number of devices and variables that must be considered, while creating an enormous communication overhead. To address this, we (1) introduce a causality filter based on Markov blankets (MB) that limits the number of variables that each device must track, (2) evaluate SLOs decentralized on a device basis, and (3) infer optimal device configuration for fulfilling SLOs. We evaluated our methodology by analyzing video stream transformations and providing device configurations that ensure the Quality of Service (QoS). The devices thus perceived their environment and acted accordingly -- a form of decentralized intelligence.

==> tables/challenge_summary.tex <==
\begin{table}[!t]
\centering
\caption{Summary of the challenges \rewrite{for a federated data sharing platform}}\label{tab:Summary_of_Challenges}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|p{14cm}|c|}
\hline
\textbf{ID} &
  \textbf{Description} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Life-cycle \\ phase\end{tabular}} \\ \hline
\textbf{C1} &
  \textit{shared metadata model} -- A domain-specific metadata model to aid the discovery and matching of data products. &
  \multirow{4}{*}{Onboarding} \\ \cline{1-2}
\textbf{C2} &
  \textit{policy language} -- Usage of a sufficiently powerful policy language to enable platform-supported lawful and trustworthy data exchange. &
   \\ \cline{1-2}
\textbf{\tmi{C3}} &
  \textit{data control plane} -- A control plane enabling domain experts to specify and update policies as data changes. &
   \\ \cline{1-2}
\textbf{C4} &
  \textit{stretched data lake} -- A policy-based data placement approach utilizing storage and streaming across federated resources &
   \\ \hline
\textbf{C5} &
  \textit{federated data catalog} -- ensure that all members of the federation can discover all data products &
  \multirow{5}{*}{Publishing} \\ \cline{1-2}
\textbf{C6} &
  \textit{consistent metadata} -- keeping browsable metadata (e.g., policies, number of records) in sync with the data product &
   \\ \cline{1-2}
\textbf{C7} &
  \textit{matchmaking} -- support the aligning and matching of consumer requirements to product metadata &
   \\ \cline{1-2}
\textbf{C8} &
  \textit{context-aware discovery} -- support interactive negotiation queries for consumer-specific metadata, based on products policy and the consumer's access purpose and context &
   \\ \cline{1-2}
\textbf{C9} &
  \textit{consumer transformations} -- support required consumer transformations, e.g., ensuring format capabilities, storage policy needs &
   \\ \hline
\textbf{C10} &
  \textit{shared agreements} -- ensure that agreements are available, immutable, in a standardized format &
  \multirow{3}{*}{Sharing} \\ \cline{1-2}
\textbf{C11} &
 \textit{enforceable agreements} -- support codifying agreement policies in an unequivocal, automatically enforceable way &
   \\ \cline{1-2}
\textbf{C12} &
 \textit{trust mechanisms} -- ensure or prove bilateral compliance with accepted agreements (e.g., monetary incentives~\cite{sober_blockchain-based_2022} or trustworthy transformations~\cite{2021_heiss_ICSOC_trustworthy}) &
   \\ \hline
\textbf{\tmi{C13}} &
  \textit{data lineage} -- enforcing and capturing agreed-upon consumption contexts, purposes, and transformations &
  \multirow{3}{*}{Consumption} \\ \cline{1-2}
\textbf{C14} &
  \textit{on-demand transformations} -- support smart and on-demand transformations to comply with policies, i.e. allocation of computations within the federation &
   \\ \cline{1-2}
\textbf{C15} &
  \textit{\rewrite{shared} access control} -- support fitting access control mechanisms, compatible with policies and execution environments &
   \\ \hline
\textbf{\tmi{C16}} &
  \textit{enforceable deletions} -- support the deletion of all copies of a data product, possibly including derivatives &
  \multirow{3}{*}{Discontinue} \\ \cline{1-2}
\textbf{C17} &
  \textit{observable lifecycle actions} -- support the audit of all data consumption actions to find and discontinue a data product &
   \\ \cline{1-2}
\textbf{\tmi{C18}} &
  \textit{\rewrite{Discontinue but leverage knowledge}} -- Keep functions and system optimization decisions for future improvement. &
   \\ \hline
\end{tabular}
}
\end{table}

==> tables/challenge_summary_v2.tex <==
\begin{table}[!t]
\centering
\caption{Summary of the challenges for a federated data exchange platform}\label{tab:Summary_of_Challenges}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|P{2.5cm}|P{10.5cm}|c|}
\hline
\textbf{ID}        & \textbf{Challenge}                                    & \textbf{Description}                                                                                                                                                                            & \textbf{\begin{tabular}[c]{@{}c@{}}Lifecycle \\ phase\end{tabular}} \\ \hline
\textbf{C1}        & \textit{Shared metadata model}                        & A domain-specific metadata model to aid the discovery and matching of federated data products                                                                                                            & \multirow{4}{*}{Onboarding}                                          \\ \cline{1-3}
\textbf{C2}        & \textit{Policy language}                              & Usage of a sophisticated policy language to enable platform-supported lawful and trustworthy data exchange                                                                             &                                                                      \\ \cline{1-3}
\textbf{C3}  & \textit{Data control plane}                           & A control plane enabling domain experts to specify and update policies as data changes                                                                                                       &                                                                      \\ \cline{1-3}
\textbf{C4}        & \textit{Stretched data lake}                          & A policy-based data placement approach utilizing storage and streaming across federated resources                                                                                               &                                                                      \\ \hline
\textbf{C5}        & \textit{Federated data catalog}                       & Ensure that all members of the federation can discover all federated data products                                                                                                                        & \multirow{5}{*}{Publishing}                                          \\ \cline{1-3}
\textbf{C6}        & \textit{Consistent metadata}                          & Keeping browsable metadata (e.g., policies, number of records) in sync with the federated data product                                                                                                    &                                                                      \\ \cline{1-3}
\textbf{C7}        & \textit{Matchmaking}                                  & Support the aligning and matching of consumer requirements to product metadata                                                                                                                  &                                                                      \\ \cline{1-3}
\textbf{C8}        & \textit{Context-aware discovery}                      & Support interactive negotiation queries for consumer-specific metadata, based on product policies, consumer's access purpose, and context                                                  &                                                                      \\ \cline{1-3}
\textbf{C9}        & \textit{Consumer transformations}                     & Support required consumer transformations, e.g., ensuring format capabilities, storage policy needs                                                                                             &                                                                      \\ \hline
\textbf{C10}       & \textit{Shared agreements}                            & Ensure that agreements are available in a standardized and immutable format                                                                                                                       & \multirow{3}{*}{Sharing}                                             \\ \cline{1-3}
\textbf{C11}       & \textit{Enforceable agreements}                       & Support codifying agreement policies in an unequivocal, automatically enforceable way                                                                                                           &                                                                      \\ \cline{1-3}
\textbf{C12}       & \textit{Trust mechanisms}                             & Ensure or prove bilateral compliance with accepted agreements (e.g., monetary incentives~\cite{sober_blockchain-based_2022} or trustworthy transformations~\cite{2021_heiss_ICSOC_trustworthy}) &                                                                      \\ \hline
\textbf{C13} & \textit{Data lineage}                                 & Enforcing and capturing agreed-upon consumption contexts, purposes, and transformations                                                                                                         & \multirow{3}{*}{Consumption}                                         \\ \cline{1-3}
\textbf{C14}       & \textit{On-demand transformations}                    & Support smart and on-demand transformations to comply with policies, i.e. allocation of computations within the federation                                                                      &                                                                      \\ \cline{1-3}
\textbf{C15}       & \textit{Federated access control}              & Support fitting access control mechanisms, compatible with policies and execution environments                                                                                                  &                                                                      \\ \hline
\textbf{C16} & \textit{Enforceable deletions}                        & Support the deletion of all copies of a federated data product, possibly including derivatives                                                                                                            & \multirow{3}{*}{Discontinue}                                         \\ \cline{1-3}
\textbf{C17}       & \textit{Observable lifecycle actions}                 & Support the audit of all data consumption actions to find and discontinue a federated data product                                                                                                        &                                                                      \\ \cline{1-3}
\textbf{C18} & \textit{Maintain knowledge} & Preserve functions and system optimization for future improvement                                                                                                                        &                                                                      \\ \cline{1-4}
\end{tabular}
}
\vspace{-1em}
\end{table}
